Can't make an Omelette without Breaking some Eggs: Plausible Action Anticipation using Large Video-Language Models

We introduce PlausiVL, a large video-language model for anticipating action sequences that are plausible in the real-world. While significant efforts have been made towards anticipating future actions, prior approaches do not take into account the aspect of plausibility in an action sequence. To address this limitation, we explore the generative capability of a large video-language model in our work and further, develop the understanding of plausibility in an action sequence by introducing two objective functions, a counterfactual-based plausible action sequence learning loss and a long-horizon action repetition loss. We utilize temporal logical constraints as well as verb-noun action pair logical constraints to create implausible/counterfactual action sequences and use them to train the model with plausible action sequence learning loss. This loss helps the model to differentiate between plausible and not plausible action sequences and also helps the model to learn implicit temporal cues crucial for the task of action anticipation. The long-horizon action repetition loss puts a higher penalty on the actions that are more prone to repetition over a longer temporal window. With this penalization, the model is able to generate diverse, plausible action sequences. We evaluate our approach on two large-scale datasets, Ego4D and EPIC-Kitchens-100, and show improvements on the task of action anticipation.

==> sec/0_abstract.tex <==
\begin{abstract}
% In this work, we introduce a \visllm which can leverage temporal information efficiently for the task of action anticipation. Recently, significant efforts have been made to accurately anticipate the future actions. However, such approaches do not consider the aspect of generating action sequences that are plausible in the real-world. To develop such understanding, we focus on two important aspects: 1) Building the ability to understand the temporal correlations among the actions that make the action sequence temporally plausible, 2). Being able to learn diverse and less repetitive actions in the future. For this, we propose a \visllm based approach and train the method with two objective functions - a counterfactual-based plausible action sequence learning loss and a long-horizon action repetition loss. The plausible action sequence learning loss helps the model understand the temporally plausible nature of actions and the long-horizon action repetition loss helps the model generate diverse actions. We validate our algorithm on two large-scale datasets, Ego4D and \epickitchens and show improvements on the task of action anticipation.

We introduce PlausiVL, a \visllm for anticipating action sequences that are plausible in the real-world. While significant efforts have been made towards anticipating future actions, prior approaches do not take into account the aspect of plausibility in an action sequence. To address this limitation, we explore the generative capability of a \visllm in our work and further, develop the understanding of plausibility in an action sequence by introducing two objective functions, a counterfactual-based plausible action sequence learning loss and a long-horizon action repetition loss. We utilize temporal logical constraints as well as verb-noun action pair logical constraints to create implausible/counterfactual action sequences and use them to train the model with plausible action sequence learning loss. This loss helps the model to differentiate between plausible and not plausible action sequences and also helps the model to learn implicit temporal cues crucial for the task of action anticipation. The long-horizon action repetition loss puts a higher penalty on the actions that are more prone to repetition over a longer temporal window. With this penalization, the model is able to generate diverse, plausible action sequences. We evaluate our approach on two large-scale datasets, Ego4D and \epickitchens, and show improvements on the task of action anticipation.


% . For developing the understanding of plausibility in our model, we focus on two important characteristics in a model: 1) Building the ability to understand the temporal correlations among the actions that make the action sequence temporally plausible, 2) Being able to learn diverse and less repetitive actions in the future. 



% 1) Building the ability to understand the temporal correlations among the actions that make the action sequence temporally plausible, 2). Being able to learn diverse and less repetitive actions in the future. For this, we propose a \visllm based approach and train the method with two objective functions - a counterfactual-based plausible action sequence learning loss and a long-horizon action repetition loss. The plausible action sequence learning loss helps the model understand the temporally plausible nature of actions and the long-horizon action repetition loss helps the model generate diverse actions. We validate our algorithm on two large-scale datasets, Ego4D and \epickitchens and show improvements on the task of action anticipation.

% First, it has to learn the underlying temporal structure of the sequence of actions that humans perform in the real world and not hallucinate. Second, language models tend to repeat text, whereas, for the task of action anticipation, the model should be able to predict the longer, temporal window of actions with diverse but temporally plausible actions. 


\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
%\let\thefootnote\relax\footnote{Work done during internship at Honda Research Institute, USA.}
\begin{figure}[t]
    \centering
    \includegraphics[trim=1.5cm 1cm 9.2cm 0cm, clip, width=\linewidth]{figures/Plausvl_final4.pdf}
    \caption{We present a \visllm for learning to anticipate action sequences that are \textit{plausible} in the real-world. We show an example of a kitchen-based environment. By using a \visllm, we leverage their generative capabilities to anticipate future actions and further train the model with two devised objective functions: plausible action sequence learning loss and long-horizon action repetition loss. Without the plausible action sequence learning loss, the model has less temporal understanding and generates a temporally implausible action sequence of \textcolor{red}{\textit{cook omlette} $\not \rightarrow$ \textit{crack eggs}}. Similarly, without the long-horizon action repetition loss, the model generates less diverse actions and repeats the same action, \textcolor{red}{\textit{whisk eggs} $\rightarrow$ \textit{whisk eggs} $\rightarrow$ \textit{whisk eggs}}. When training the model with the two objective functions combined, our method is able to generate plausible action sequences which are temporally accurate, \textcolor{Green}{\textit{crack eggs} $\rightarrow$ \textit{cook omlette}} and more diverse with less repetition, \textcolor{Green}{\textit{whisk eggs} $\rightarrow$ \textit{whisk eggs} $\rightarrow$ \textit{cook omlette}}.}
    \vspace{-4mm}
    \label{fig:intro_diagram}
\end{figure}

Having the ability to predict future events is a critical component in the decision-making process of an AI agent. For example, for an autonomous driving car, being able to anticipate the next sequence of actions for cars, pedestrians, and other agents in the scene can ensure safety of pedestrians as well as vehicles. To enable this, the model should be able to reason effectively from the spatial as well as temporal information of the visual scene. This has led to a growing interest in the task of \textit{Action Anticipation}. Action anticipation refers to the predictive task of forecasting future actions or activities given a sequence of visual data, typically videos. 
%is the task where given the current state of the environment, the agent should be able to predict the next sequence of actions that might occur in the environment.
For example, in a kitchen-based environment, if a human has performed the following series of actions, \textit{open fridge} $\rightarrow$ \textit{take eggs} $\rightarrow$ \textit{close fridge}, the model should be able to reason that \textit{crack eggs} could be one of the plausible future actions.

However, action anticipation is challenging because the uncertainty in precisely predicting the future makes the task non-deterministic in nature. In other words, given what has happened so far, there are infinitely many possibilities for what future actions might happen. Moreover, action anticipation is accompanied by an additional challenge of understanding the implicit temporal information present in an action sequence, which makes the sequence \textit{plausible} in the real-world. For example, the model should be able to understand that an action like \textit{crack eggs} will always happen \textit{\textbf{before}} \textit{cook omelette} as shown in Figure~\ref{fig:intro_diagram}. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[trim=1.5cm 1cm 9.2cm 0cm, clip, width=\linewidth]{figures/Plausvl_final4.pdf}
%     \caption{We present a \visllm for learning to anticipate \textit{plausible} future action sequences by optimizing two objective functions: plausible action sequence learning loss and long-horizon action repetition loss. We show an example of a kitchen-based environment where the person takes eggs from the fridge, cracks the eggs, and whisks the eggs. Without the plausible action sequence learning loss, the model has less temporal understanding and generates a temporally implausible action sequence of \textit{cook omlette} $\rightarrow$ \textit{crack eggs}. }
%     \label{fig:intro_diagram}
% \end{figure}

% should have a strong understanding of temporal nature of an action sequence which makes it \textit{plausible} in the real-world over a long horizon. 

To this end, there has been some progress for the action anticipation task. Earlier works have explored an LSTM based approach by summarizing the past and inferring the future~\cite{furnari2020rolling, osman2021slowfast}, by logging the past history actions in text~\cite{manousaki2023vlmah}, or using RNN-based approaches~\cite{roy2022predicting, shi2018action} by learning goals. However, such LSTM/RNN-based approaches are unable to effectively capture the temporal relations among the actions over a long horizon due to their sequential nature. There have been efforts to resolve this limitation by implementing different types of attention mechanism~\cite{gong2022future}, skip-connection~\cite{ke2019time}, and message-passing framework~\cite{tai2022unified}. However, they show marginal improvement in modeling longer horizon. Recent works have also explored transformer-based approaches~\cite{girdhar2021anticipative, gong2022future, roy2022interaction}, with a memory-based system~\cite{wu2022memvit} or leveraging multiple-modalities~\cite{zhong2023anticipative,zhang2023object}. While transformer-based approaches are able to model longer temporal understanding, they can still become confined to the information present in the training data and cannot model the diverse nature of the future actions. They rely on the ability of the transformer encoder to learn from the given training data which limits their generalization and scaling capability.
% they are encoder-based and their classifier, and the existing approaches have to fine-tune the entire backbone which has limitations in scalability.
% Owing to the success of leveraging language models to transform image recognition into generative tasks, we propose  as a generative/completion task. 
% using an auto-regressive text generation LLM model for action anticipation. 
% Some recent methods have tried to leverage gen llm for vision tasks by harnessing autoreg text gen ability for improving generalization. taking inspiration and addresses the challenges to anticipate plausible actions, we propose plausivlm which can do so and so.
% \textbf{TODO: limitation of these transformer approaches} 

% \textbf{TODO: need to fill the gap that where LSTM, rnn, transformer failed and why llm is helpful}

% A strong understanding of temporal information is especially necessary to understand the intent and end goal from the past action sequence.

To overcome the above challenges, recent methods~\cite{li2023blip,alayrac2022flamingo,wang2023all,li2023lavender} have attempted to leverage the autoregressive text generation capabilities of generative large-language models~(LLMs) to improve generalizability for various vision tasks. Taking inspiration from these works and to address the challenges present in anticipating plausible actions, we introduce \textbf{\method}, \textbf{Plausi}ble action anticipation through a large \textbf{V}ideo-\textbf{L}anguage model. 

Given the generative capabilities of large language models, in this work, we introduce a video-large-language model which can efficiently model and leverage the temporal cues present in a video to generate plausible action sequences for the task of action anticipation. We use a Q-former~\cite{li2023blip} based transformer architecture to embed videos into spatio-temporal visual representations. This architecture ensures an effective alignment between the visual features and the desired text in the LLM embedding space. In addition to the alignment, we try to address the challenges that are specifically present in the task of action anticipation and thus, introduce a method with the following important characteristics: 1). The ability to understand the temporal correlations present among the actions in a sequence which in turn makes the action sequence temporally \textit{plausible} in the real-world, 2). Being able to model the diverse, possible actions that can happen in the future. For example, for the former characteristic, a model should follow a temporal constraint that \textit{an action X has to happen before for the action Y to happen} to make the sequence \textit{action X} $\rightarrow$ \textit{action Y} plausible in the real-world.

To build such temporal understanding required for generating plausible action sequences, we design a counterfactual-based plausible action sequence learning loss where we create temporal logic constraints and train the model to be able to differentiate between the plausible and not plausible action sequences. Additionally, we also use verb-noun action logical constraints to further improve the model's understanding about which verbs are possible with which nouns to create a plausible action in the real-world~(for example, cook spoon is not a plausible action). To our knowledge, the aspect of plausibility in generating an action sequence has not been explored for the task of action anticipation. While this loss is helpful for efficient temporal understanding, we also aim for the model to be able to understand the diverse nature of actions and generate plausible action sequences with less repeated actions as language models are prone to the issue of repetition. To resolve this, we devise a long-horizon action repetition loss where the later actions that are more prone to repetition have a higher penalty and the earlier, immediate actions have lower penalty. We summarize our contributions as follows:

\begin{enumerate}
    \item We present \method, a \visllm which leverages the spatial-temporal information present in videos for anticipating plausible future action sequences.
    \item To learn the temporal cues and understand the temporal dependencies among actions in a plausible sequence, we design a counterfactual-based plausible action sequence learning loss. We create temporal logic rules and verb-noun action pair logic constraints for the model to be able to understand plausibility in action sequences.
    \item To be able to generate less diverse future actions with less repetition, we devise a long-horizon action repetition loss by penalizing the longer-horizon actions more.  
\end{enumerate}

% While a simple approach is to give a text prompt to the language model to anticipate the future actions, simply using text prompts for downstream tasks creates a loss of crucial information that is present in the visual modality. Such text-based approaches/models especially cannot understand the real-world, temporal flow of actions, interactions with objects in an environment, and the temporal dynamics of the real-world. Hence, in this work, we propose a method to utilize videos to efficiently capture the visual as well as temporal information present in them. 


% While this module ensures an efficient video-text alignment for LLMs, we   to address the challenges that are specifically present in the task of action anticipation due to the following reasons: 1) a model should be able to leverage the temporal cues that are essentially needed to generate a \textit{plausible} sequence of action, 2). Since language models are prone to the issue of repetition and such models may not be able to model the diversity present in the future actions.

 % There have been recent approaches~\cite{chen2023videollm,zhang2023video} that have leveraged videos to achieve efficient video-text alignment, however, simply using these methods to anticipate future actions can still fail due to the following two reasons: 1) They are unable to leverage the temporal cues that are essentially needed to generate a \textit{plausible} sequence of action, 2) Language models are prone to the issue of repetition and such models may not be able to model the diversity present in the future actions. Such \visllm models~\cite{chen2023videollm,zhang2023video} are prone to failures as they are unable to learn the highly diverse temporal dependencies and correlations among the actions over long horizons. 
 
 % For example, a \visllm would fail to model the temporal logic constraint that \textit{an action X has to happen before an action Y} as they are designed to optimize only the language modelling loss. A language modelling loss cannot model such type of implicit information in the ground truth sequence of action. 
 
 % To build the temporal understanding required for generating \textit{plausible} action sequences, we use a counterfactual-based plausible action sequence learning loss where we create temporal logic constraint: \textit{an action X that has to happen before an action Y}. Such logical constraints would help the model to differentiate between plausible and not plausible action sequences. We also use verb-noun action logical constraints to further improve the model's understanding about which verbs are possible with which nouns to create a plausible action. While this loss is helpful for efficient temporal understanding, language models suffer from the issue of repetition and fail to model the diverse nature of future actions. To resolve this, we propose a long-horizon action repetition loss where the later actions that are more prone to repetition have a higher penalty and the earlier actions have lower penalty. The objective function has not been explored for the task of action anticipation. We summarize our contributions as follows:

% \begin{enumerate}
%     \item We explore the potential of \visllm based approach for the task of action anticipation.
%     \item To leverage the temporal cues for the task of action anticipation, we propose a counterfactual-based plausible action sequence learning loss.
%     \item To mitigate the issue of repetition in language models, we devise a long-horizon action repetition loss.
% \end{enumerate}


% Good Notes
% Recent work on large language models\textbf{TODO:add citations} use text prompt for various downstream tasks like question-answering, \textbf{TODO:add more tasks}, etc. However, such approaches only operate in a textual space and are at a loss of important information that is present in the visual modality. To mitigate this issue, there have been recent efforts~\cite{li2023blip}\textbf{TODO:add citations} towards visual-language alignment to bring the visual modality closer to the textual space of large language model so that the large language model can understand and infer from visual modality. However, these approaches are focused mainly on static images and cannot be easily extended for the task of action anticipation which is heavily conditioned on the temporal information underlying in a sequence of actions. To leverage the temporal information, Additionally, language models are also prone to \textit{repetition} and may fail to generate a long-range sequence of future actions.



% \textbf{TODO: write/sell this better}To this end, we present our work which uses a \visllm-based approach to predict the future actions. While models like \visllm are able to generate semantic actions, they are unable to learn the highly diverse temporal dependencies and corrrelations among the actions over long horizons. For example, a \visllm would fail to model the temporal logic constraint that \textit{an action X has to happen before an action Y} as they are designed to optimize only the language modelling loss. A language modelling loss cannot model such type of implicit information in the ground truth sequence of action. 


% What work has been done?
% What they lack?
% What we do?
% What we propose?

% Currently, we have witnessed the potential of textual large language models in multiple applications. At the same time,  Works like brings the image modality closer to the language model space. At the same time, there are ongoing efforts for the video modality. With this, we pose the question, can a large language model learn to anticipate the future action using visual modality?





==> sec/2_related_works.tex <==
\section{Related Works}
\label{sec:related_works}

% \begin{figure*}[t]
%     \centering
%     \includegraphics[trim=0.2cm 8cm 2.5cm 3cm, clip, width=\linewidth]{figures/model_diagram_a7.pdf}
%     \includegraphics[trim=1.4cm 0cm 1.2cm 0.1cm, clip, width=\linewidth]{figures/model_diagram_bc7.pdf}
%     \vspace{-5mm}
%     \caption{\textbf{Model diagram:(a) \method}: Given a video of $N$ frames, a frozen visual encoder is used to extract frame level representations which are passed through a Q-former with $k$ number of query tokens and concatenated with a frame position embedding layer to add temporal understanding. Next, they are passed through the video Q-former to get spatio-temporal representations and a linear layer is added to project these features into the LLM space. These visual embeddings are considered as soft prompts and are concatenated with the text-prompt to get the desired output~(Section~\ref{sec:model_architecture}), \textbf{(b). Augmentation:} For the model to be able to generate plausible action sequences, we use logical counterfactual rules to create implausible action sequences. Given an input video, we create a positive augmentation of the video by color jitter, etc. and a negative augmentation by using temporal logical constraints and verb-noun pair action constraints~(Section~\ref{sec:Lplau}). \textbf{(c). Objective Functions and Training:} We train our model with two losses: Plausible Action Sequence Learning Loss~($\Lplau$) which aligns the original video-plausible text pair closer to the positive augmentation of video-plausible text, and brings the original video-plausible text far apart from the video-counterfactual text.~(Section~\ref{sec:Lplau}), long-horizon action repetition loss that helps the model to generate diverse and less repetitive actions by adding a higher penalty to the later tokens~(mix mixture and wipe hands) and lower penalty to immediate future actions~(pour water, pour water). The graph shows the linearly increasing $\gamma$ penalty for the tokens over the long-horizon~(Section~\ref{sec:Lrep}).}
%     \label{fig:model_diagram}
% \end{figure*}

\textbf{Large Language Models.}
Language Modeling is a method to model the generative likelihood over the word token sequences and predict the probabilities of the next/future tokens. Large language models~(LLMs)~\cite{brown2020language,chowdhery2022palm,taylor2022galactica,touvron2023llama} are transformers with billions of parameters that have been trained on massive amounts of data and have shown impressive capabilities on the task of question-answering and chat-conversation with humans. Methods like in-context learning~\cite{brown2020language}, prompt tuning~\cite{white2023prompt}, chain-of-thought reasoning~\cite{wei2022chain}, and reinforcement learning with human feedback~\cite{ouyang2022training,christiano2017deep} have improved the language models to perform very well on few-shot tasks. While these models show great capabilities in understanding the input and solving complex tasks via text generation, these models can only understand the text modality and are at a loss of the rich information that is present in other modalities like video, audio. In our work, we utilize videos as input and learn from the visual and temporal information present in them.

\noindent \textbf{Large Vision-Language Models.} %Vision Language Models (VLMs) mark a significant convergence in artificial intelligence, aiming to unify visual comprehension with natural language understanding.  
Recent strides in this domain have seen diverse pre-training methods leveraging extensive multimodal datasets driving the progress of large vision-language models. Some models~\cite{radford2021learning, jia2021scaling, furst2022cloob, li2021supervision, wang2023protege} merge visual and linguistic modalities by co-training text and image encoders using contrastive loss on large datasets containing image-caption pairs. Meanwhile, other approaches~\cite{alayrac2022flamingo, chen2022visualgpt} integrate visual input directly into language model decoders through a cross-attention mechanism, eschewing the use of images as additional prefixes. Another category of vision-language models~\cite{li2019visualbert, lu2019vilbert, chen2020uniter, singh2022flava, tan2019lxmert, li2020oscar} leverage Masked-Language Modeling (MLM) and Image-Text Matching (ITM) objectives to align image segments with text.
%There have been ongoing efforts~\cite{alayrac2022flamingo} to align the visual and text modalities so that the LLMs can understand and infer from the visual modality. 
BLIP-2~\cite{li2023blip} was one of the works which proposed a Qformer-based method to ensure visual-text alignment. Since these works explore the image-text alignment, they are unable to model and understand the temporal information that is present in videos. There have been efforts towards video-text alignment by using a linear layer to project the video space to the LLMs textual space~\cite{chen2023videollm} in Video-LLM or by using a Q-former based module~\cite{zhang2023video} in Video-LLaMA. While these works explore video-text alignment, these models can be ineffective for the task of action anticipation as they do not understand the temporal correlations among the actions in a sequence.

\noindent \textbf{Temporal and symbolic logic reasoning.} Symbolic logic reasoning is a method to create a system of rules and symbols in the form of logical expressions. Temporal logic reasoning specifically designs logical expressions for representing and reasoning about time. Linear temporal logic~\cite{pnueli1977temporal}, metric temporal logic~\cite{montanari1996metric}, signal temporal logic~\cite{fainekos2009robustness}, and interval temporal logic~\cite{halpern1991propositional} are some methods for develop temporal logical rules. We take inspiration from the work DTL~\cite{xu2022don} to generate temporal logic rules and create counterfactual sequences of actions.

\noindent \textbf{Action Anticipation.}
%For the task of action anticipation, given a video V with T frames, the video is passed through a backbone network which generates the future anticipation actions in the form of verb-noun pairs. 
This task has been explored for third-person videos~\cite{vondrick2016anticipating,abu2018will,gao2017red,chen2022gatehub,rizve2023pivotal} as well as egocentric videos~\cite{rodin2022untrimmed, qi2021self, girdhar2021anticipative, furnari2022towards, damen2018scaling, damen2020rescaling, grauman2022ego4d}. Standard approaches for this task can be divided into LSTM/RNN-based~\cite{shi2018action, damen2020rescaling} approaches and transformer-based approaches. LSTM-based approaches~\cite{furnari2020rolling, osman2021slowfast} mainly use a rolling LSTM to encode the observed video and store an updated summary. For inference, an unrolling LSTM is initialized with the hidden and cell state of the rolling LSTM to predict the next action. While LSTM/RNNs have shortcomings in modeling long-horizon temporal dependencies, some approaches mitigate this issue via goal-based learning~\cite{roy2022predicting}, diverse attention mechanism~\cite{gong2022future}, skip-connections~\cite{ke2019time}, message passing framework~\cite{tai2022unified}, memory-based modules~\cite{wu2022memvit, manousaki2023vlmah} or similarity metric~\cite{fernando2021anticipating}. Recent works have explored transformer-based~\cite{girdhar2021anticipative, grauman2022ego4d} approaches with global attention~\cite{gong2022future}, modelling apperance change in human-object interactions~\cite{roy2022interaction}, conditioning on intention~\cite{mascaro2023intention}, hierarchical feature aggregation~\cite{mascaro2023intention}. While most of the works explore it in a unimodal setting by using the visual modality, other works also present a multi-modal approach for this task by using optical flow~\cite{furnari2020rolling,osman2021slowfast}, object-based features~\cite{furnari2020rolling,osman2021slowfast,zhang2023object} or audio~\cite{mittal2022learning,zhong2023anticipative}. Other works explore uncertainty-based methods~\cite{furnari2018leveraging, abu2019uncertainty} and GAN-based approach~\cite{gammulle2019predicting}. We take inspiration from the object detection~\cite{lin2017focal} literature for the repetition loss. Concurrent to our work, there have been text-based LLM approaches~\cite{zhao2023antgpt,huang2023palm} which explore the task of action anticipation, however, they only operate in the textual space and lose the visual-temporal information present in video.


% All text must be in a two-column format.
% The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
% Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
% The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
% The second and following pages should begin 1 inch (2.54 cm) from the top edge.
% On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
% for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
% page.

% %-------------------------------------------------------------------------
% \subsection{Margins and page numbering}

% All printed material, including text, illustrations, and charts, must be kept
% within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
% high.
% %
% Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
% The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
% The \LaTeX\ template takes care of this when used properly.



% %-------------------------------------------------------------------------
% \subsection{Type style and fonts}

% Wherever Times is specified, Times Roman may also be used.
% If neither is available on your word processor, please use the font closest in
% appearance to Times to which you have access.

% MAIN TITLE.
% Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
% The title should be in Times 14-point, boldface type.
% Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
% do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
% Leave two blank lines after the title.

% AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
% and printed in Times 12-point, non-boldface type.
% This information is to be followed by two blank lines.

% The ABSTRACT and MAIN TEXT are to be in a two-column format.

% MAIN TEXT.
% Type main text in 10-point Times, single-spaced.
% Do NOT use double-spacing.
% All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
% Make sure your text is fully justified---that is, flush left and flush right.
% Please do not place any additional blank lines between paragraphs.

% Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
% Short captions should be centred.

% \noindent Callouts should be 9-point Helvetica, non-boldface type.
% Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

% FIRST-ORDER HEADINGS.
% (For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

% SECOND-ORDER HEADINGS.
% (For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
% If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

% %-------------------------------------------------------------------------
% \subsection{Footnotes}

% Please use footnotes\footnote{This is what a footnote looks like.
% It often distracts the reader from the main flow of the argument.} sparingly.
% Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
% If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
% Use Times 8-point type, single-spaced.


% %-------------------------------------------------------------------------
% \subsection{Cross-references}

% For the benefit of author(s) and readers, please use the
% {\small\begin{verbatim}
%   \cref{...}
% \end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
% This will automatically insert the appropriate label alongside the cross-reference as in this example:
% \begin{quotation}
%   To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
%   It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
%   You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
% \end{quotation}
% If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
% {\small\begin{verbatim}
%   \Cref{...}
% \end{verbatim}}
% command. Here is an example:
% \begin{quotation}
%   \Cref{fig:onecol} is also quite important.
% \end{quotation}

% %-------------------------------------------------------------------------
% \subsection{References}

% List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
% When referenced in the text, enclose the citation number in square brackets, for
% example~\cite{Authors14}.
% Where appropriate, include page numbers and the name(s) of editors of referenced books.
% When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
% If you use the template as advised, this will be taken care of automatically.

% \begin{table}
%   \centering
%   \begin{tabular}{@{}lc@{}}
%     \toprule
%     Method & Frobnability \\
%     \midrule
%     Theirs & Frumpy \\
%     Yours & Frobbly \\
%     Ours & Makes one's heart Frob\\
%     \bottomrule
%   \end{tabular}
%   \caption{Results.   Ours is better.}
%   \label{tab:example}
% \end{table}

% %-------------------------------------------------------------------------
% \subsection{Illustrations, graphs, and photographs}

% All graphics should be centered.
% In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
% Instead use
% {\small\begin{verbatim}
%   \centering
% \end{verbatim}}
% at the beginning of your figure.
% Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
% Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
% Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
% You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

% When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
% {\small\begin{verbatim}
%    \usepackage{graphicx} ...
%    \includegraphics[width=0.8\linewidth]
%                    {myfile.pdf}
% \end{verbatim}
% }


% %-------------------------------------------------------------------------
% \subsection{Color}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

% If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
% Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_method.tex <==
\vspace{-1mm}
\section{Method}
\label{sec:method}
\begin{figure*}[t]
    \centering
    % \includegraphics[trim=0.2cm 8cm 2.5cm 3cm, clip, width=0.95\linewidth]{figures/model_diagram_a7.pdf}
    % \includegraphics[trim=1.4cm 0cm 1.2cm 0.1cm, clip, width=0.95\linewidth]{figures/model_diagram_bc9.pdf}
    \includegraphics[trim=2.5cm 8cm 2.5cm 3cm, clip, width=0.9\linewidth]{figures/model_diagram_a7.pdf}
    \includegraphics[trim=3.7cm 0cm 1.2cm 0.1cm, clip, width=0.9\linewidth]{figures/model_diagram_bc9.pdf}
    \vspace{-3mm}
    \caption{\textbf{Model diagram:(a) \method}: Given a video, a frozen visual encoder a Q-former with $k$ number of query tokens is used to extract frame level representations which are further concatenated with a frame position embedding layer to add temporal understanding. Next, the representations are passed through the video Q-former and a linear layer is added to project these features into the LLM space. These visual embeddings~(visual prompts) and are concatenated with text-prompts to get the desired output text~(Sec~\ref{sec:model_architecture}), \textbf{(b) Augmentation:} For plausible action anticipation, we use logical rules to create counterfactual implausible action sequences. Given an input video, we create a positive augmentation of the video and a negative augmentation by using temporal logical and verb-noun action pair constraints~(Sec~\ref{sec:Lplau}). \textbf{(c) Objective Functions and Training:} We train our model with two losses: (i) Plausible Action Sequence Learning Loss~($\Lplau$) which aligns the original video-plausible text pair closer to the positive augmentation of video-plausible text, and brings the original video-plausible text far apart from the video-counterfactual text.~(Sec~\ref{sec:Lplau}), (ii) long-horizon action repetition loss that ensures diverse and less repetitive actions by adding a higher penalty to the later tokens~(mix mixture and wipe hands) and lower penalty to immediate future actions~(pour water, pour water). The graph shows the linearly increasing $\gamma$ penalty for the tokens over the long-horizon~(Sec~\ref{sec:Lrep}).}
    \label{fig:model_diagram}
\end{figure*}

In the following sections, we present the details of our method, \method, to learn the temporal cues for plausible action sequence generation. 
% needed for the task of action anticipation. 

% Section~\ref{sec:model_architecture} provides an overview of the architecture for learning visual representations, section~\ref{sec:training} discusses about training and the proposed objective functions that we use in our method, section~\ref{sec:Lplau} discusses about the plausible action sequence learning loss along with the constraints used in our work to create the counterfactuals. Finally, Section~\ref{sec:Lrep} discusses about the long-horizon action repetition loss and brings both the losses together.

% \subsection{Action Anticipation Task Setup}

% For the task of action anticipation, given a video V with T frames, $V = \{v_{1}, v_{2}, v_{3}..., v_{t}\}$, the video is passed through a backbone network which generates the $N$ future anticipation actions in the form of verb-noun pairs, $A = \{(v_{1}, n_{1}), (v_{2}, n_{2}), .....(v_{N}, n_{N})\}$. 

% \textbf{Ego4D~\cite{grauman2022ego4d}:} Given a video $V$ and a stopping time $t$, the model predicts $N$ sets of sequences having $Z$ number of actions in the form of verb-noun pairs, $\{\{(\hat{v}_{z, n}, \hat{n}_{z, n})\}^{Z}_{z=1}\}_{n=1}^N$, where, $\hat{v}_{z, n}$ is the predicted verb and $\hat{n}_{z, n}$ is the predicted noun. \newline

% \noindent \textbf{\epickitchens~\cite{damen2020rescaling}:} For this dataset, given an action segment that starts at time $\tau_{s}$, the model has to predict the anticipated action by observing a video segment of duration $[\tau_{s} - (\tau_{o} + \tau_{a}), \tau_{s} - \tau_{a}]$ where $\tau_{o}$ is the observation time and $\tau_{a}$ is the anticipation time. The anticipation time $\tau_{a}$ means how much in advance the model has to anticipate the action.  

% a video segment of duration $\tau_{o}$~(observation time) and ending $\tau_{a}$~(anticipation time) seconds before the action's start time, is given to the model to generate the next future action in the form of verb-noun pair, $(\hat{v}_{t}, \hat{n}_{t})$. Referring to , the model observes a video segment  to predict the next action.

\subsection{Model Architecture}
\label{sec:model_architecture}
Given a video clip of $N$ frames, $V = [v_{1}, v_{2}, v_{3}....v_{N}]$, we use a frozen visual encoder~(ViT) to extract video-frame-level representations, $V = [v'_{1}, v'_{2}, v'_{3}....v'_{N}]$. After this, each frame feature is passed through a Q-former~\cite{li2023blip} with $k$ number of query tokens, to get the $d_q$-dimensional visual representation as $v''_{i}\in\mathbb{R}^{k \times d_{q}}$. These queries are helpful in extracting the visual features with the most information aligned to the text. For the frames to have an understanding of the temporal relations among them, a frame position embedding layer is applied to each Q-former feature. At the same time, we also apply a clip-position embedding layer to infuse more grouping information about the frames that belong to a clip. These features are then passed through a video Q-former to aggregate the spatio-temporal information of the video. Finally, a linear projection layer is used to project these output representations to the LLM text embedding space of $d_l$ dimension, $v_{i}\in\mathbb{R}^{k_{l} \times d_{l}}$. These video embeddings can be considered as \textit{visual prompts} which are concatenated with the input text embeddings $t_i$ to make the LLM generate text conditioned on the video content. 

% where $v'_{i}\in\mathbb{R}^{K_{f} \times d_{f}}$. After this, a position embedding layer is used to encode temporal information into the video frames which is then passed through a video Q-former~\cite{li2023blip} to aggregate the frame and temporal information and get $k_v$ video embedding vectors of dimension $d_v$, $\hat{v}\in\mathbb{R}^{k_{v} \times d_{v}}$. Finally, a linear layer is used to project these output representations to the LLM text embedding space, $v_{i}\in\mathbb{R}^{k_{l} \times d_{l}}$. These visual embeddings are used as a \textit{soft visual prompt} and are concatenated with the input LLM text embeddings, $t_i$ to make the frozen LLM generate text that is conditioned on the video content. Video-LLM operates on both the visual and auditory modality. In our framework, we only use the visual branch of Video-LLaMA.
% In this work, we use the video $V$ as our input and a text prompt $P$ to query the visual large-language model.

\section{Training}
\label{sec:training}
While the above backbone network ensures the alignment of the visual features with the LLM textual space, we also focus on making the model learn to better understand long-horizon temporal dependencies among the actions which is crucial for plausible action anticipation. To develop such temporal understanding in a model, we train our system to optimize two losses, (1). Plausible Action Sequence Learning loss $\Lplau$ and (2). Long-horizon action repetition loss $\Lrep$. With these two losses, the model can understand the temporal cues better to be able to generate a \textit{plausible} and diverse sequence of future actions.

\vspace{-2mm}
\subsection{Plausible Action Sequence Learning loss}
\label{sec:Lplau}
% While a language modelling loss is helpful for text generation, a \visllm with only language modelling loss has less understanding of the temporal dependencies and correlations that are present among the actions. 
For a model to be able to understand the plausible nature of an action sequence, it should be able to leverage the implicit temporal information present in input videos. Thus, we design a self-supervised plausible action sequence learning loss, $\Lplau$. The key idea is to create counterfactuals based on temporal logical constraints as well as verb-noun action pair logical constraints and optimize the network by minimizing a loss with two negative log-likelihood terms: (1) \textit{increase} the probability of associating the visual modality with the temporally correct and plausible sequence of actions, and (2) \textit{decrease} the probability of associating the video with the action sequences that are not plausible in the real-world and temporally incorrect. Here, sequences of action that satisfy the temporal as well as verb-noun action pair logic constraints are considered as logically correct.

\noindent \textbf{Temporal logical constraints}: In our work, we define a temporal constraint for an action sequence as follows: \textit{an action X that has to happen before an action Y} to make it a plausible sequence in the real-world. \noindent Consider for example, given a sequence of \textit{take eggs} $\rightarrow$ \textit{crack eggs} $\rightarrow$ \textit{whisk eggs} $\rightarrow$ \textit{cook omelette}, a counterfactual of this sequence of actions would be, \textit{take eggs} $\rightarrow$ \textit{cook omelette} $\rightarrow$ \textit{whisk eggs} $\rightarrow$ \textit{crack eggs} since \textit{crack eggs} would always happen before \textit{cook omelette}. Mathematically, we define it as follows:
% \begin{align}
%     T_{(a_i, a_j)} = \forall_{(a_i, a_j) \in \mathbb{D}} (a_i \rightarrow a_j) \wedge \neg (a_j \rightarrow a_i) 
% \end{align}
\begin{align}
\small
    CF^{temp}(a_i, a_j) = \begin{dcases*}
        1, & if $ \forall_{t \in T} (t_{a_i} \rightarrow t_{a_j}) \wedge \neg (t_{a_j} \rightarrow t_{a_i}),  $ \\
        -1 & if $ \forall_{t \in T} (t_{a_j} \rightarrow t_{a_i}) \wedge \neg (t_{a_i} \rightarrow t_{a_j}),  $ \\
        0, & otherwise. 
        \end{dcases*}
\end{align}
\noindent where $CF^{temp}(a_i, a_j)$ is an action pair matrix with a value of 1 if $a_i$ always happens before $a_j$ for all the ground truth sequences $t \in T$, a value of -1 if $a_i$ always happens after $a_j$, and 0 otherwise if there is no relation between the two actions. With this temporal logical constraint, given a text sequence $t$, we perform a swap operation if there is a forward or backward relation between an action pair. Hence, given a ground truth text sequence $t$, we define the operation if $a_j$ always happens before $a_p$ as follows:
\begin{align}
\small
    t^{cf}(a_i, a_j, a_p, a_n) = \begin{dcases*}
        a_i, a_p, a_j, a_n, & if $ CF^{temp}(a_j, a_p)=1,  $ \\
        a_i, a_j, a_p, a_n, & otherwise. 
        \end{dcases*}
\end{align}
\noindent Similarly, we define the operation if $a_j$ always happens after $a_i$ as follows:
\begin{align}
\footnotesize
    t^{cf}(a_i, a_j, a_p, a_n) = \begin{dcases*}
        a_j, a_i, a_p, a_n, & if $CF^{temp}(a_j, a_i)=-1,$ \\
        a_i, a_j, a_p, a_n, & otherwise. 
        \end{dcases*}
\end{align}
\noindent Next, we define the another logical constraint - verb-noun action pair constraint. 

% \kwon{Define $\mathbb{D}$. In the previous paragraph, the example is on 3 actions. How is it related to the equation which contains 2 actions?}
\noindent \textbf{Verb-Noun Action pair constraints}: For this, we create a counterfactual where a verb-noun action pair is not plausible in the real-world, for example, \textit{cook spoon}. We define a verb-noun action constraint as follows: \textit{a verb-noun pair consisting of an action verb that is plausible with the object noun} in the real-world. Mathematically, we define it as follows: 
\begin{align}
    CF^{act}(a_i, a_j) = \begin{dcases*}
        1, & if $ \forall_{t \in T} \neg ({a^v_i} \wedge {a^n_j}),  $ \\
        0, & otherwise. 
        \end{dcases*}
\end{align}
\noindent where $CF^{act}(a_i, a_j)$ is a verb-noun pair matrix with a value of 1 if for a verb, the corresponding noun is not plausible or vice-versa in all the ground truth actions $t \in T$ and 0 otherwise if the verb-noun pair is plausible. Similar to the temporal constraints mentioned above, with this verb-noun action pair constraint, given an action, we swap either the verb or noun with a uniform probability to create implausible verb-noun action pairs. Given a text action pair $t$, we define the operation of a counterfactual, implausible verb-noun action pair as follows:
\begin{dmath}
    t^{cf}(a^v_i, a^n_i) = \begin{dcases*}
        (a^v_i, a^n_j) || (a^v_j, a^n_i), & if $ CF^{act}(a^v_i, a^n_j) = 1,  $ \\
        (a^v_i, a^n_i), & otherwise. 
        \end{dcases*}
\end{dmath}
\noindent \textbf{Loss:} With this, for every video-text action sequence pair $(V_i, T_i)$ in the dataset $\mathcal{D}$, we create a temporal as well as verb-noun action pair counterfactual $T^{cf}_i$ for every textual ground truth text sequence and collect it as a dataset, $\mathcal{D}_{vtcf}$. Finally, we define plausible action sequence learning loss~($\Lplau$) as follows:
\begin{dmath}
	\Lplau = \mathbb{E}_{(v_i, t_i) \in \mathcal{D}_{\mathtt{vtcf}}}\biggl[
	- \log \Bigl(z(v_i, t_i, v'_i)\Bigr)
	- \log \left(1 - z(v_i, t_i, t^{cf}_i)\right)\biggr]
	\label{eq:Lplau}
\end{dmath}
\noindent In the above equation, $z(v_i, t_i, v'_i)$ and $z(v_i, t_i, t^{cf}_i)$ probabilities are computed as follows:
\begin{align}
    \centering
    z(v_i, t_i, v'_i) &= \sigma\Bigl(\mathtt{sim}( \Delta p(v_i, t_i), \Delta p(v'_i, t_i) )/ \tau\Bigr) \\
    z(v_i, t_i, t^{cf}_i) &= \sigma\left(\mathtt{sim}( \Delta p(v_i, t_i), \Delta p(v_i, t^{cf}_i) )/ \tau\right)
\end{align}
\noindent where $v_i$ and $v'_i$ are the visual embeddings of the original video and augmented video~(respectively), $t_i$ and $t^{cf}_i$ are the text embeddings of the ground truth text sequence and counterfactual text~(respectively), $\tau$ is the temperature, $\sigma$ is the sigmoid function, $\Delta p(., .)$ is the cross-modal video-text representation from LLM after passing through a MLP projection layer~(absorbed in the equation for better readability), and $\mathtt{sim}$ is the similarity function. \newline

\noindent In summary, training the model to optimize the $\Lplau$ loss helps the model to differentiate between the plausible and counterfactual/implausible action sequences by aligning the visual modality closer to the temporally correct, plausible action sequence. By learning this alignment, it is able to understand the implicit temporal information that defines the dependencies and correlations among actions in a plausible sequence.


% \begin{figure}[t]
%     \centering
%     \includegraphics[trim=0 14cm 14cm 0, clip, width=\linewidth]{figures/ek100_anticipation.pdf}
%     \vspace{-5mm}
%     \caption{\textbf{Action Anticipation Task Setup:} For \epickitchens, given an action segment starting at time $\tau_s$, the model observes a video segment of length $\tau_o$ and anticipates the future action that happens $\tau_a$ seconds in advance}
%     \label{fig:ek100anticipation}
% \end{figure}

% \noindent where $p(v_i, t_i)$ is the probability computed from the similarity of $v_i$ and ground truth text $t_i$, and $p(v_i, t^{cf}_i)$ is the probability computed from the similarity of $v_i$ and counterfactual text $t^{cf}_i$.  


% \begin{align}
%     \centering
%     p(v_i, t_i) &= \sigma\left(\mathtt{sim}(v_i, t_i)/ \tau\right) \\
%     p(v_i, t^{cf}_i) &= \sigma\left(\mathtt{sim}(v_i, t^{cf}_i)/ \tau\right)
% \end{align}

\subsection{Long-Horizon Action Repetition Loss}
\label{sec:Lrep}
While the plausible action sequence learning loss $\Lplau$ helps the model to understand the implicit temporal information present in the action sequences, we consider another aspect of plausibility by reducing the repetition of actions and in turn generating more diverse actions. We observe that while the model is able to generate accurate, temporally correct, and diverse actions over a short temporal window, it starts repeating the same actions over a longer horizon. To mitigate this, we train the model by enforcing a larger penalty on the actions that happen over a longer horizon in the temporal window and lesser penalty to the actions that are immediately near to the observed video. We add a penalty of $\gamma_t$ over the negative log-likelihood of the probability as follows:
\begin{align}
    \centering
    p_t &= \frac{\exp(\hat{y}_t)}{\Sigma_j \exp(\hat{y}_j)}, \\
    \Lrep(p_t) &= -{\gamma_t}log(p_t)
    \label{eqn:Lrep}
\end{align}
\noindent where $\hat y_t$ is the output from the language model for the $t$'th token over which softmax operation is applied to get the probability $p_t$. $\gamma_t$ is the $\gamma$ value temporally unique to the $t$'th token following the order, ${\gamma_0} < {\gamma_1} < {\gamma_2} < \cdots < {\gamma_N}$.

\noindent In summary, by optimizing the $\Lrep$ loss, the model is penalized more for the actions that happen over a longer horizon and less penalized for immediate actions. This is helpful in regulating repetition and ensuring more diverse actions in the generated text. 

\noindent Finally, we train our model with the overall loss as:
\begin{equation}
    \centering
    \mathcal{L} = \alpha\Lplau + \beta\Lrep
    \label{eqn:bothlosses}
\end{equation}
\noindent where $\alpha$ and $\beta$ are the weight hyper-parameter for the two losses. 

% You must include your signed IEEE copyright release form when you submit your finished paper.
% We MUST have this form before your paper can be published in the proceedings.

% Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
% \url{https://www.computer.org/about/contact}.

==> sec/4_experiments.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Implementation Details}
We process the videos of size $224 \times 224$ with Ego4D containing 8 clips with 4 frames, making a total of 32 frames, and \epickitchens with 32 frames as well. We use the pretrained Qformer model, BLIP2-FlanT5xxl from BLIP2~\cite{li2023blip} with number of query tokens as 32 and ViT-G/14 as our vision encoder. We train our method end-to-end with a learning rate of $1e^{-5}$, for 100 epochs, and $\alpha = 0.5$ and $\beta = 0.5$. We use LLaMA-2-7B as our language model. For long-horizon action repetition loss, $\Lrep$, we use $\gamma$ in the uniform distribution from $[0, 2]$ with number of steps equal to the number of output tokens from the language model. For plausible action sequence learning loss $\Lplau$, we use video augmentation of color jitter, random horizontal flip, and a random rotation of 10 degrees.

\subsection{Experimental Setup}

\noindent \textbf{Datasets:} We evaluate on two action anticipation datasets: Ego4D~\cite{grauman2022ego4d} and \epickitchens~\cite{damen2020rescaling}. Ego4D is a large-scale egocentric dataset covering diverse indoor and outdoor scenarios like home, workplace, etc. It consists of 3670 hours of videos with 115 verbs and 478 nouns. To evaluate our method on Ego4D, we use videos from the Forecasting and Hand-Object interaction subset and show results on the validation set. In Ego4D, a video and a stopping time is given, and the model predicts $N$ sets of sequences having $Z$ number of actions in the form of verb-noun pairs, $\{\{(\hat{v}_{z, n}, \hat{n}_{z, n})\}^{Z}_{z=1}\}_{n=1}^N$, where, $\hat{v}_{z, n}$ is the predicted verb and $\hat{n}_{z, n}$ is the predicted noun. 

\noindent \epickitchens~\cite{damen2020rescaling} is an egocentric dataset of a kitchen-based environment. It consists of 100 hours of egocentric videos with 97 verbs and 300 nouns. For this dataset, given an action segment that starts at time $\tau_{s}$, the model has to predict the anticipated action by observing a video segment of duration $[\tau_{s} - (\tau_{o} + \tau_{a}), \tau_{s} - \tau_{a}]$ where $\tau_{o}$ is the observation time and $\tau_{a}$ is the anticipation time. The anticipation time $\tau_{a}$ means how much in advance the model has to anticipate the action. 

\noindent \textbf{Baselines:} We compare our method with \visllms, Video-LLaMA~\cite{zhang2023video} and Video-LLM~\cite{chen2023videollm}. We also compare our method with the transformer and LSTM-based approaches for action anticipation along with text-based large language models for a more exhaustive analysis.

\noindent \textbf{Ablation Study:} In the ablation study, we present results of \method with and without $\Lplau$ and $\Lrep$ objective functions to show the effect of each component on the final performance of the model.

% \input{tables/ego4d_ek100_maintable}
\input{tables/main_ego4d}
\input{tables/main_ek100}
\input{tables/ablation_ego4d_ek100}
\input{tables/bleu_repetition}
% \input{tables/ablation_ego4D}

\subsection{Discussion of Results}
Referring to Table~\ref{tbl:mainego4d} and Table~\ref{tbl:mainek100}, we can observe that \method is able to perform better when compared with the baselines. This can be attributed to its ability to be able to understand the plausibility in the action sequences and leverage the temporal correlations among the actions in a sequence. We present a closer analysis of the results in our discussion following next.

\noindent \textbf{\method shows performance gain towards action anticipation:} Prior \visllms~\cite{zhang2023video,chen2023videollm} have only explored the visual-text alignment and lack the temporal understanding needed for the action anticipation. To show that our model is able to learn the temporal understanding, we compare \method with Video-LLM and Video-LLaMA in Table~\ref{tbl:mainego4d} and observe an improvement of 4.2\% and 2.4\%, respectively on verbs. Similarly, we observe an improvement of 2.72\% and 2.22\% on verbs for \epickitchens in Table~\ref{tbl:mainek100}. The improvement in the performance emphasizes that the model is able to learn the temporal dependencies among the actions to generate more accurate and plausible action sequences. Qualitative results presented in Figure~\ref{fig:qual_results} also show the quality of our generated sequence in comparison to the ground truth. We can see that our method is able to understand the activity happening the video and anticipate the temporal future action sequence accordingly. We also exhaustively compare \method with prior approaches in Table~\ref{tbl:mainego4d} and Table~\ref{tbl:mainek100} that utilize transformer and LSTM-based architectures and show that our method is able to perform better. 

\noindent \textbf{$\Lplau$ helps the model to learn plausible future action sequences:} We hypothesize that for generating accurate future action sequences, a model should have an understanding about the temporal plausibility of an action sequence in the real-world. To assess if our devised loss function, plausible action sequence learning loss, $\Lplau$ is able to create such understanding in the model, we compare our method, row (1) and our method without $\Lplau$, rows (3) and (4) in Table~\ref{tbl:ablationego4dek100}. We observe by removing this module, there is a drop in the performance of 1.2~\% on verbs for Ego4D and 1.47~\% for verbs of \epickitchens~(row(1) and row(3) are compared). This shows that training a model with $\Lplau$ as an objective function helps the model to learn the implicit temporal information of action correlations in a sequence. Through learning to differentiate between the plausible and not plausible action sequences and aligning the video representations closer to the plausible action sequences, the model learns an effective video-text alignment which helps in generating more accurate, plausible future action sequences.
% Moreover, by seeing the counterfactual implausible action sequences during training, it is able to implicitly understand the temporal cues needed for the task of action anticipation.
\begin{figure*}[t]
    \centering
    \includegraphics[trim=0cm 4.5cm 0cm 0cm, clip, width=0.95\linewidth]{figures/qual_results4.pdf}
    \vspace{-5mm}
    \caption{Qualitative Results: Given a video, the top \textcolor{blue}{blue} box shows the prediction from \method and the \textcolor{Green}{green} box contains the ground truth action sequence for reference. We can observe that \method is able to generate action sequences that satisfy the temporal logic constraints and are diverse with less repetitions. The predicted action sequence is also closer to the ground truth action sequence.}
    \label{fig:qual_results}
    \vspace{-4mm}
\end{figure*}
% While a \visllm is able to anticipate actions, we observe that a \visllm  is unable to understand the temporal dependencies among the actions in a sequence to make it a plausible sequence. To assess if $\Lplau$ is helping the model to generate plausible action sequences, we compare our method with~(\textbf{Row}) and without $\Lplau$~(\textbf{Row}) in Table~\ref{tbl:ablationego4dek100}. We can observe that training the model with $\Lplau$ helps with the performance by \textbf{TODO}. This shows that by using temporal as well as action pair constraints and training the model with counterfactual does help the model to understand and differentiate between the plausible and not plausible action sequences. By aligning the video representations closer to the plausible action sequence and taking the video representations away from not plausible action sequences, the model is able to understand that what makes a sequence plausible and not plausible and is also able to understand the temporal correlations among actions needed for the task of action anticipation. 

\noindent \textbf{$\Lrep$ helps with lesser repetition and more diversity over long horizons:} We also try to address another aspect of plausibility in action sequences by making the model learn to generate sequences with less repetitive actions and more diverse actions via our devised objective function, long-horizon action repetition loss, $\Lrep$. To assess the efficacy of this module, we compare our method, row (1) and our method without $\Lrep$, row (2) and row (4) in Table~\ref{tbl:ablationego4dek100}. We observe that there is performance dip of 1.5~\% on Ego4D nouns and 0.63~\% on \epickitchens nouns. This indicates that by penalizing the actions more over the long horizon, $\Lrep$ is able to reduce the repetition of actions in the sequence generation and hence, contribute towards plausible action anticipation sequences.
% helping the model to generate more accurate action anticipation sequences by reducing the repetition of actions in the sequence generation. By penalizing the actions over a longer horizon more than the immediate future actions, the module is helping towards more accurate action anticipation.

% We also try to address the issue of repetition in the generated sequences from a \visllm by training the model via $\Lrep$. When comparing rows \textbf{TODO} and \textbf{TODO} in Table~\ref{tbl:ablationego4dek100}, we can observe that training with $\Lrep$ makes the performance even better. This indicates the objective function is helping the model to generate more accurate action anticipation sequences by reducing the repetition in the long-horizon sequence generation. It penalizes the actions over a longer horizon more than the immediate future actions and is thus helping towards more accurate action anticipation. 
\noindent \textbf{\Visllm vs Text-large-language-model:} Given the exploration of text-only large language models, we also address the comparison between text-based LLM and \visllms for the task of action anticipation. We compare \method with AntGPT~\cite{zhao2023antgpt} which is a text-based LLM and observe a performance gain of 2.1\% on verbs and 3.6\% on nouns for Ego4D from our method. We reason that a major drawback of text-based LLM for this task is that they completely discard the visual as well as temporal information present in the videos. Whereas, the task of action anticipation is highly dependent on the visual spatio-temporal information to understand the real-world temporal flow of actions and anticipate actions accurately. Incorporating visual modality can give crucial information such as the environment of the agent, the objects interacted with, and other objects in the scene which might be interacted with later in the future. Such vital information is lost when converting a video into textual actions~\cite{zhao2023antgpt} or into a summary~\cite{huang2023palm}. Summarizing a video into text-based information can only provide the high-level details about a video, but it doesn't give a signal about the real-world temporal flow of the actions and objects in a video.

% \noindent \textbf{\method is able to generate plausible action sequences:} To further analyze the quality of the generated text from \method and emphasize the plausibility and less repetition in our generated text, we compute the BLEU score. The BLEU score measures the similarity between our generated text and ground truth. We report the results in Table~\ref{tbl:bleurep}. By having a better BLEU score than the baseline, we show that the generated text is a more plausible action sequence which emphasizes the efficacy of our objective functions. Moreover, a lower edit distance metric in Table~\ref{tbl:mainego4d} also indicates less repetition and more plausibility in the generated text as a lower metric would mean less substitutions were made to bring the output text closer to the ground truth.

% with repetition score and BLEU score
\noindent \textbf{\method is able to generate plausible action sequences:} To further emphasize the plausibility, less repetition and quality our generated text, we compute the BLEU score~\cite{papineni2002bleu} and repetition score. The repetition score is an average of the number of actions that are repeated in an action sequence and the BLEU score measures the similarity between our generated text and ground truth. We report the results in Table~\ref{tbl:bleurep}. By having a better BLEU score than the baseline, we show that the generated text from our method is a more plausible action sequence, thus emphasizing the efficacy of our objective functions. Similarly, by having a lower repetition score than the baseline, we show that the model has lesser repetitive actions in the generated sequence. Our method repeats 5.87 actions in an action sequence on average whereas Video-LLaMA repeats an average of 7.12 actions. We also observe an average repetition of 4.33 actions in ground truth action sequences. Moreover, a lower edit distance metric in Table~\ref{tbl:mainego4d} also indicates less repetition and more plausibility in the generated text as a lower metric would mean less substitutions were made to bring the output text closer to the ground truth.





==> sec/5_conclusion.tex <==
\vspace{-2mm}
\section{Conclusion}
\label{sec:conclusion}
\vspace{-2mm}
In this work, we leverage the generative capabilities of \visllms for plausible action anticipation. In addition to the abilities of \visllms, for the model to better understand the plausibility in an action sequence, we introduce a plausible action sequence learning loss which helps the model to differentiate between the plausible and not plausible action sequences, and thus learn anticipation related temporal cues. We further devise a long-horizon action repetition loss that puts a higher penalty on the actions that happen over a longer temporal window and are more prone to repetition, thus mitigating action repetition and ensuring more diverse actions. Experimental results show that our model is able to perform better by generating more plausible and accurate action sequences on Ego4D and \epickitchens. While our method is an initial step towards plausible action anticipation, there can be further exploration mitigating the issue of hallucinating implausible action sequences in the future work. 

% In this work, we leverage the generative capabilities of \visllms for plausible action anticipation. In addition to this, for the model to better understand the plausibility in an action sequence, we introduce a plausible action sequence learning loss which helps the model to differentiate between the plausible \& not plausible action sequences, and thus learn anticipation related temporal cues. We further devise a long-horizon action repetition loss that puts a higher penalty on the actions that happen over a longer temporal window and are more prone to repetition, thus mitigating action repetition and ensuring more diverse actions. Experimental results show that our model is able to perform better by generating more plausible and accurate action sequences. While our method is a step towards plausible action anticipation, there can be further exploration mitigating the issue of hallucination of implausible action sequences in the future work. 

% In this work, we explored the potential \visllms for the task of action anticipation. The main question we tried to explore is if a \visllm can understand and leverage the temporal cues needed to understand the correlations among the actions over a long horizon and hence, perform well on the task anticipation. While a \visllm is able to generate the textual actions, it falls short of two aspects: generating temporal sequence of actions that are plausible in the real-world and repetition of the actions over a long horizon. We address these two aspects by proposing by a plausible action sequence learning loss and a long-horizon action repetition loss. The plausible action sequence loss aligns the visual modality closer to the plausible temporal action sequence and far from the not plausible action sequence. Whereas, the long-horizon action repetition loss assigns a higher penalty to the tokens that are at a longer horizon that the tokens that are near/immediate to the observed video. Experimental results show that by training our \visllm with these two objective functions, our model is able to perform better on the task of action anticipation. While our method is a step towards generating plausible and diverse future action sequences, there can be exploration mitigating the issue of hallucinating not plausible action sequences and repeating the same actions over a long horizon in the future work. 

==> sec/X_suppl_camera_ready.tex <==
% \clearpage
% \setcounter{page}{1}
% \maketitlesupplementary

\section{Implementation Details}
We train our method end-to-end with a batch size of 2 for Ego4D and 4 for \epickitchens, linear warmup cosine as learning rate scheduler, along with the pre-trained weights of Video-LLaMA~\cite{zhang2023video} on 2 A6000 GPUs for 2.5 days.  

\subsection{Metrics}
\textbf{Edit Distance~(ED@(Z=20))~\cite{grauman2022ego4d}:} This metric is computed over a sequence of verb and noun predictions using the Damerau-Levenshtein distance~\cite{damerau1964technique,levenshtein1966binary} and takes into account the sequential nature of the action anticipation task. A prediction is considered correct if it matches the ground truth at a specific time step using the edit distance operations - insertion, deletion, substitution, and transposition. A total of $K$ predictions are evaluated and the smallest edit distance between a prediction and ground truth is reported~\cite{grauman2022ego4d}. We consider the value of $Z=20$ and $K=5$ which is the same as Ego4D~\cite{grauman2022ego4d}. \newline

\noindent \textbf{Class-mean Top-5 Recall~(\%)~\cite{damen2020rescaling}:} This metric evaluates if the ground truth class is within the top-5 predictions and averages the per-class performance to equally weight all the classes. The top-k criterion takes into account the uncertainty/multi-modality in the future action prediction and class-mean is helpful for balancing the long-tail distribution.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/graph.png}
    \vspace{-5mm}
    \caption{Analysis of plausibility in generated action sequence: \textcolor{black}{Black} line represents our method and \textcolor{orange}{orange} is the baseline, Video-LLaMA. Comparing the two line plots, we can observe that \method follows more number of temporal and action constraints over training than Video-LLaMA indicating that the objective functions $\Lplau$ and $\Lrep$ are helping the model to learn temporal cues needed to generate plausible action sequences for action anticipation.}
    \label{fig:constraint_graph}
\end{figure}


\section{Quantitative Analysis}

\textbf{Generalization and robustness to long-tail:} We evaluate our method on the unseen participants and tail classes of \epickitchens~\cite{damen2020rescaling} and present the results in Table~\ref{tbl:unseentailek100}. Unseen participants consists of those participants that are not present in the train set and tail classes are defined to be the smallest classes whose instances are around 20\% of the total number of instances in the train set. We observe that a better performance of our approach on the unseen participants as compared to the other baselines shows the generalizability of our model across unseen data. Similarly, a better performance on the tail classes shows that our model is robust to the long-tail distribution of the \epickitchens dataset. \newline

\input{tables/unseen_tail_ek100}
\input{tables/supp_dnr_ego4d}
\input{tables/supp_dnr_ek100}
\input{tables/suppreb_repetition_analysis}
\input{tables/suppreb_clr_loss}



% \noindent \textbf{Quality of the generated text:} To assess the aspect of plausibility and less repetition in the generated text, we compute the Shannon entropy of our model and compare it with the baseline, Video-LLaMA in Table~\ref{}. A better shannon entropy than the baseline shows that the losses, $\Lplau$ and $\Lrep$ are helpful in improving the quality of the text and bringing the generated text closer to the ground truth text, hence making the text more plausible along with less repetition. \newline

\noindent \textbf{Analysis of plausibility in generated action sequence:} To evaluate if the generated text is a plausible action sequence and additionally, the efficacy of the $\Lplau$ and $\Lrep$ objective functions, we calculate the average number of temporal and action constraints followed in the generated text. We compare the average number of constraints followed by \method versus the baseline Video-LLaMA~\cite{zhang2023video} and present the graph visualization in Figure~\ref{fig:constraint_graph}. We report the average number of constraints followed over the training and show the number over the checkpoints from beginning till the end of training. From the figure, we can observe that as the training of the model with $\Lplau$ and $\Lrep$ losses progresses, the average number of constraints followed increases in the generated text. Morever, the average number of \method is higher than that of Video-LLaMA. This indicates that by training the model with $\Lplau$ and $\Lrep$ objective functions, the model can generate more plausible action sequences and they help the model learn the implicit temporal information needed for plausible action anticipation. \newline

\noindent \textbf{Training with $\Lrep$ loss vs prompt tuning:} We perform an analysis where instead of training the model with $\Lrep$ objective function, we simply prompt the model with the phrase: "Do NOT repeat actions"~(DNR). We compare \method trained with $\Lplau$ and $\Lrep$ losses~(row 2) and \method trained with $\Lplau$ and DNR prompt~(row 1) and present the results of this analysis for Ego4D in Table~\ref{tbl:dnr_ego4d} and for \epickitchens in Table~\ref{tbl:dnr_ek100}. We can observe that simply prompting the model with DNR in the prompt does not give much improvement in the performance as compared to training the model with long-horizon action repetition loss~($\Lrep$) as objective function. Training the model $\Lrep$ penalizes the model for repeating the actions and makes the model learn to generate more diverse actions. This penalty is helpful in reducing repetition of the actions over a long-horizon. Simply stating DNR in the prompt only gives an instruction/command to the model, whereas, training the model with $\Lrep$ loss influences the learning of the model which is needed for the task of action anticipation. \newline

\noindent \textbf{$\Lrep$ loss is dataset independent}: We perform an analysis to highlight that repetition loss is independent of the dataset. In other words, the performance of the repetition loss does not depend on the number of repeated actions in a dataset. We present this analysis in Table~\ref{tbl:suppreb_rep_analysis}. We observe no strong correlation between n\_rep and performance, showing data-independency and also show that \method w/ repetition loss reduces repetition and outperforms the baseline. \newline

\noindent \textbf{Different videos as negative samples for $\Lplau$ loss:} For the $\Lplau$ loss, we use an implausible action sequence as a negative sample. We perform an analysis of using negative samples from other videos and show the results in Table~\ref{tbl:r2_clr}. This setting performs worse than Row 2,3 as it gives a weaker signal of counterfactual temporal plausibility than the signal of an implausible action sequence, since sequences from other videos are also temporally plausible. \newline

\noindent \textbf{Anticipation time $\tau_a$ vs Accuracy:} 
$\tau_a$ is the anticipation time between the end time of observed video and the starting time of the first action to be anticipated. The video during the anticipation period $\tau_a$ is unobserved. For EK100, $\tau_a$=1s and for Ego4D, $\tau_a$=2.20s on an average. We analyze changing $\tau_a$ versus accuracy on EK100 in Figure~\ref{fig:taua_accuracy}. We can observe that the method is quite robust till $\tau_a$=3.5s whereas Video-LLaMA is only robust till $\tau_a$=2.0s for EK100. This shows that the model can predict future actions even with a far anticipation time.


\begin{figure}[t]
    \centering
    \includegraphics[trim=0.2cm 0.2cm 0.3cm 0.3cm, clip, width=0.93\linewidth]{figures/graph_draft6.png}
    \caption{Analysis of $\tau_a$ vs. verb-noun class-mean Top-5 recall (\%) accuracy on EK100~$\uparrow$.}
    \label{fig:taua_accuracy}
\end{figure}

% \input{tables/supp_postprocess_ego4d}
% \input{tables/supp_postprocess_ek100}

% \noindent \textbf{Using constraints as post-processing instead of training with $\Lplau$:} In this analysis, we emphasize the importance of plausible action sequence learning loss~($\Lplau$). We compare our model's output when trained with $\Lplau$ vs our model when trained without $\Lplau$ and with post-processed output using the temporal constraints. In post processing, the positions of the actions in the generated sequences is switched/swapped to make the sequence temporally plausible. We present the results on Ego4D in Table~\ref{tbl:postprocess_ego4d} and \epickitchens in Table~\ref{tbl:postprocess_ek100}. We can observe that post processing the output with constraints does not give much improvement in the performance~(row 1). Whereas, training the model with $\Lplau$ significantly helps with the performance on both Ego4D and \epickitchens. This is because training the model with $\Lplau$ helps the model to learn implicit temporal cues that are needed for the task of action anticipation. Having a better temporal understanding in turn helps the model to generate action sequences that are plausible in the real-world. With post processing on the output, the model cannot leverage such temporal cues present in the videos. \newline

\begin{figure*}[t]
    \centering
    \includegraphics[trim=0cm 4.5cm 0cm 0cm, clip, width=0.93\linewidth]{figures/supp_fig1.pdf}
    \includegraphics[trim=0cm 3.5cm 0cm 0cm, clip, width=0.93\linewidth]{figures/supp_fig2.pdf}
    \includegraphics[trim=0cm 3.5cm 0cm 0cm, clip, width=0.93\linewidth]{figures/supp_fig3.pdf}
    \vspace{-6mm}
    \caption{Qualitative Results over videos of diverse environments like kitchen, construction sites, etc. and their respective anticipated actions from our method. Given a video, the top \textcolor{blue}{blue} box shows the prediction from \method and the \textcolor{Green}{green} box contains the ground truth action sequence for reference. The model is able to generate plausible action sequences.}
    \label{fig:supp_qual_results1}
\end{figure*}


\section{Qualitative Analysis}
In this section, we present more qualitative results of our method. Given a video, the top \textcolor{blue}{blue} box shows the prediction from \method and the \textcolor{Green}{green} box contains the ground truth action sequence for reference. We can observe that 
our method is able to understand the activity happening in the video and then, generate action sequences accordingly. Additionally, \method is able to generate action sequences that satisfy the temporal logic constraints and are diverse with less repetitions. The predicted action sequence is also closer to the ground truth action sequence.





==> sec/method_orig.tex <==
\section{Preliminaries}
\label{sec:method}

\subsection{Action Anticipation Task Setup}

% For the task of action anticipation, given a video V with T frames, $V = \{v_{1}, v_{2}, v_{3}..., v_{t}\}$, the video is passed through a backbone network which generates the $N$ future anticipation actions in the form of verb-noun pairs, $A = \{(v_{1}, n_{1}), (v_{2}, n_{2}), .....(v_{N}, n_{N})\}$. 

\textbf{Ego4D~\cite{grauman2022ego4d}:} Given a video $V$ and a stopping time $t$, the model predicts $N$ sets of sequences having $Z$ number of actions in the form of verb-noun pairs, $\{\{(\hat{v}_{z, n}, \hat{n}_{z, n})\}^{Z}_{z=1}\}_{n=1}^N$, where, $\hat{v}_{z, n}$ is the predicted verb and $\hat{n}_{z, n}$ is the predicted noun, as shown in Figure~\ref{}. \newline

\noindent \textbf{\epickitchens~\cite{damen2020rescaling}:} For this dataset, given an action segment that starts at time $\tau_{s}$, the model has to predict the anticipated action by observing a video segment of duration $[\tau_{s} - (\tau_{o} + \tau_{a}), \tau_{s} - \tau_{a}]$ where $\tau_{o}$ is the observation time and $\tau_{a}$ is the anticipation time. The anticipation time $\tau_{a}$ means how much in advance the model has to anticipate the action~(Figure~\ref{fig:ek100anticipation}).  

% a video segment of duration $\tau_{o}$~(observation time) and ending $\tau_{a}$~(anticipation time) seconds before the action's start time, is given to the model to generate the next future action in the form of verb-noun pair, $(\hat{v}_{t}, \hat{n}_{t})$. Referring to , the model observes a video segment  to predict the next action.

\subsection{Video-LLaMA~\cite{zhang2023video}}
Video-LLaMA is a LLM-based framework which processes a multi-modal video to be able to chat with humans. It builds upon the architecture of BLIP-2~\cite{li2023blip}. Given a video of $N$ frames, it uses a frozen pre-trained visual encoder~(ViT~\&~Qformer) to extract video-frame-level representations, $V = [v_{1}, v_{2}, v_{3}....v_{N}]$ where $v_{i}\in\mathbb{R}^{K_{f} \times d_{f}}$. After this, a position embedding layer is used to encode temporal information into the video frames which is then passed through a video Q-former~\cite{li2023blip} to aggregate the frame and temporal information and get $k_v$ video embedding vectors of dimension $d_v$, $\hat{v}\in\mathbb{R}^{k_{v} \times d_{v}}$. Finally, a linear layer is used to project these output representations to the LLM text embedding space. These visual embeddings are used as a \textit{soft visual prompt} and are concatenated with the input text embeddings to make the frozen LLM generate text that is conditioned on the video content. Video-LLM operates on both the visual and auditory modality. In our framework, we only use the visual branch of Video-LLaMA. \textbf{Extra lines} The Audio-language branch uses Imagebind as the frozen pre-trained audio encoder. The rest of the architecture is similar as the Video-Language Branch as described above.
% In this work, we use the video $V$ as our input and a text prompt $P$ to query the visual large-language model.

\section{Our method}
\textbf{TODO: why language modelling loss can't do action anticipation}
While Video-LLaMA is helpful in aligning the visual features to the LLM text space, it is unable to model the temporal dependencies among actions over a long-horizon that is needed for the task anticipation. To develop such temporal understanding in a model, we train our system to optimize two losses, (1). Plausible Action Sequence Learning loss $\Lplau$ and (2). Long-horizon action repetition loss $\Lrep$. With these two losses, the model can understand the temporal cues better to be able to generate a \textit{plausible} and diverse sequence of future actions. 
\textbf{TODO: change v notation and write that video and text passed through encoders and over that the losses are applied, change the loss notations}

\subsection{Plausible Action Sequence Learning loss~($\Lplau$)}
While the language modelling is helpful for text generation, a \visllm with only language modelling loss has less understanding of the temporal dependencies and correlations between the actions. \textbf{TODO} Such implicit temporal information is important to generate plausible sequence of future actions. For the model to be able to learn the temporal aspect of the future actions, we propose a self-supervised plausible action sequence learning loss, $\Lplau$. The key idea is to create counterfactuals based on temporal logical constraint as well as verb-noun action pair logic constraints and optimize the network by minimizing a loss with two negative log-likelihood terms: (1) \textit{increase} the probability of associating the visual modality with the logically correct and plausible sequence of actions, and (2) \textit{decrease} the probability of associating the video with the action sequence that is logically incorrect and not plausible in the real-world. Here, sequences of action that satisfy the temporal as well verb-noun action pair logic constraints are considered as logically correct.
\textbf{TODO: check below equation}

\begin{figure}[t]
    \centering
    \includegraphics[trim=0 14cm 14cm 0, clip, width=\linewidth]{figures/ek100_anticipation.pdf}
    \vspace{-5mm}
    \caption{\textbf{Action Anticipation Task Setup:} For \epickitchens, given an action segment starting at time $\tau_s$, the model observes a video segment of length $\tau_o$ and anticipates the future action that happens $\tau_a$ seconds in advance}
    \label{fig:ek100anticipation}
\end{figure}

\begin{equation}
\centering
	\Lplau(v_i, t_i) = \left[
	- \log \left(p(v_i, t_i)\right)
	- \log \left(1 - p(v_i, t^{cf}_i)\right)\right]
	\label{eq:Lplau}
\end{equation}

\noindent where $p(v_i, t_i)$ is the probability computed from the similarity of $v_i$ and ground truth text $t_i$, and $p(v_i, t^{cf}_i)$ is the probability computed from the similarity of $v_i$ and counterfactual text $t^{cf}_i$.  

\begin{align}
    \centering
    p(v_i, t_i) &= \sigma\left(\mathtt{sim}(v_i, t_i)/ \tau\right) \\
    p(v_i, t^{cf}_i) &= \sigma\left(\mathtt{sim}(v_i, t^{cf}_i)/ \tau\right)
\end{align}

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/model_diagram_template.pdf}
%     \vspace{-5mm}
%     \caption{\textbf{TODO} Model diagram}
%     \label{fig:model_diagram}
% \end{figure*}

\noindent \textbf{Temporal constraint counterfactual}: In our work, we define a temporal constraint for an action sequence as follows: \textit{an action X that has to happen before an action Y} to make it a plausible sequence in the real-world. \noindent Consider for example, given a sequence of \textit{crack eggs} $\rightarrow$ \textit{whisk eggs} $\rightarrow$ \textit{cook omlette}, a counterfactual of this sequence of actions would be, \textit{cook omlette} $\rightarrow$ \textit{whisk eggs} $\rightarrow$ \textit{crack eggs} since \textit{crack eggs} would always happen before \textit{cook omlette.} Mathematically, we define it as follows:

\begin{align}
    T_{(a_i, a_j)} = \forall_{(a_i, a_j) \in \mathbb{D}} (a_i \rightarrow a_j) \wedge \neg (a_j \rightarrow a_i) 
\end{align}

\noindent \textbf{Verb-Noun Action constraint counterfactual}: For this, we create a counterfactual where a verb-noun pair is not plausible in the real-world, for example, \textit{cook spoon}. We define a verb-noun action constraint as follows: \textit{a verb-noun pair consisting of an action verb that is plausible with the object noun} in the real-world. Mathematically, we define it as follows:

\subsection{Long-horizon action repetition loss~($\Lrep$)}

While the counterfactual-based contrastive learning loss $\Lplau$ helps the model to understand the implicit temporal information in action sequences, \visllm struggle from the issue of \textbf{repetition} in the generated text. Due to this, the model is unable to generate diverse actions over a long horizon. To mitigate, we train the model by enforcing a larger penalty on the actions that happen over later in the temporal window and less penalty to the actions that are near to the observed video. We add a penalty of $\gamma_t$ over the negative log-likelihood of the probability as follows:

\begin{align}
    \centering
    p_t &= \frac{\exp(\hat{y}_t)}{\Sigma_j \exp(\hat{y}_j)}, \\
    \Lrep(p_t) &= -(1 - p_t)^{\gamma_t}log(p_t)
    \label{eqn:Lrep}
\end{align}

\noindent where $\hat y_t$ is the output from the language model for the t'th token over which softmax operation is applied to get the probability $p_t$. $\gamma_t$ is the $\gamma$ value temporally unique to the t'th token.

\noindent In summary, by training the model to optimize the $\Lplau$ loss makes the model understand the implicit information of temporal dependencies and correlations among actions in a sequence.

\textbf{why this loss is needed}



\noindent In summary, by optimizing the $\Lrep$ loss, the model penalizes the actions more that happen over the longer-horizon more than the actions that happen closer to the observed video. By a larger penalty, the issue of repetition in language models gets mitigated. \newline 

\noindent Finally, we train our model with:

\begin{equation}
    \centering
    \mathcal{L} = \alpha\Lplau + (1 - \alpha)\Lrep
    \label{eqn:bothlosses}
\end{equation}

\noindent where $\alpha$ is the weight hyper-parameter for the two losses. 



% You must include your signed IEEE copyright release form when you submit your finished paper.
% We MUST have this form before your paper can be published in the proceedings.

% Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
% \url{https://www.computer.org/about/contact}.

==> tables/ego4d_ek100_maintable.tex <==
\begin{table*}[]
\centering
\begin{tabular}{lcccccc}
    &    & \multicolumn{2}{c}{\textbf{Ego4D}}                              & \multicolumn{3}{c}{\textbf{EPIC-Kitchens-100}}                                             \\ \hline
\multicolumn{1}{|c||}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Modality}}} & \multicolumn{2}{c|}{\textbf{ED@(Z=20)} $\downarrow$}                         & \multicolumn{3}{c|}{\textbf{Class-mean Top-5 recall~(\%)} $\uparrow$}                                 \\ \cline{3-7} 
\multicolumn{1}{|c||}{}                        & \multicolumn{1}{c|}{}                          & \multicolumn{1}{c}{\textbf{Verb}} & \multicolumn{1}{c|}{\textbf{Noun}}   & \multicolumn{1}{c}{\textbf{Verb}} & \multicolumn{1}{c}{\textbf{Noun}} & \multicolumn{1}{c|}{\textbf{Action}} \\ \hline
\multicolumn{1}{|l||}{\textcolor{lightgray}{AntGPT~\cite{zhao2023antgpt}}} & \multicolumn{1}{c|}{\textcolor{lightgray}{Text}}                      & \textcolor{lightgray}{0.700}                      & \multicolumn{1}{l|}{\textcolor{lightgray}{0.717}}  &  \multicolumn{1}{c}{\textcolor{lightgray}{-}}                       & \multicolumn{1}{c}{\textcolor{lightgray}{-}}                        & \multicolumn{1}{c|}{\textcolor{lightgray}{-}}      \\ \hline
\multicolumn{1}{|l||}{Video LLM~\cite{chen2023videollm}} & \multicolumn{1}{c|}{Video} & 0.721                    & \multicolumn{1}{l|}{0.725}  & \multicolumn{1}{c}{-}                        & \multicolumn{1}{c}{-}                        & \multicolumn{1}{c|}{15.40}  \\ 
\multicolumn{1}{|l||}{Video LLaMA~\cite{zhang2023video}} & \multicolumn{1}{c|}{Video}                     & \multicolumn{1}{l}{0.703} & \multicolumn{1}{l|}{0.721}       &  \multicolumn{1}{c}{52.90}                        &    \multicolumn{1}{c}{52.01}                      & \multicolumn{1}{c|}{26.05}       \\ \hline
\multicolumn{1}{|l||}{\textbf{Ours}}  & \multicolumn{1}{c|}{Video}  & \multicolumn{1}{l}{\textbf{0.679}}  & \multicolumn{1}{l|}{\textbf{0.681}}       & \multicolumn{1}{c}{\textbf{55.62}}   &  \multicolumn{1}{c}{\textbf{54.23}}   & \multicolumn{1}{c|}{\textbf{27.60}}       \\ \hline
\end{tabular}
\caption{Performance on Long-term action anticipation on Ego4D $\downarrow$: Lower is better, and \epickitchens on class-mean Top-5 recall~(\%) $\uparrow$): Higher is better}
\label{tbl:mainego4dek100}
\end{table*}



% \begin{table*}[]
% \centering
% \begin{tabular}{lcclllll}
%                                               &                                             &                                                & \multicolumn{2}{c}{\textbf{Ego4D}}                              & \multicolumn{3}{c}{\textbf{EPIC-Kitchens-100}}                                             \\ \hline
% \multicolumn{1}{|c||}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Modality}}} & \multicolumn{2}{c|}{\textbf{ED@(Z=20)} $\downarrow$}                         & \multicolumn{3}{c|}{\textbf{Class-mean Top-5 recall~(\%)} $\uparrow$}                                 \\ \cline{4-8} 
% \multicolumn{1}{|c||}{}                        & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                          & \multicolumn{1}{c}{\textbf{Verb}} & \multicolumn{1}{c|}{\textbf{Noun}}   & \multicolumn{1}{c}{\textbf{Verb}} & \multicolumn{1}{c}{\textbf{Noun}} & \multicolumn{1}{c|}{\textbf{Action}} \\ \hline
% \multicolumn{1}{|l||}{\textcolor{lightgray}{AntGPT~\cite{zhao2023antgpt}}}                  & \multicolumn{1}{l|}{\textcolor{lightgray}{LLaMA2-7B}}                       & \multicolumn{1}{c|}{\textcolor{lightgray}{Text}}                      & \textcolor{lightgray}{0.700}                      & \multicolumn{1}{l|}{\textcolor{lightgray}{0.717}}  &  \multicolumn{1}{c}{\textcolor{lightgray}{-}}                       & \multicolumn{1}{c}{\textcolor{lightgray}{-}}                        & \multicolumn{1}{c|}{\textcolor{lightgray}{-}}      \\ \hline
% % \multicolumn{1}{|l||}{\textcolor{lightgray}{Palm~\cite{huang2023palm}}}                    & \multicolumn{1}{l|}{\textcolor{lightgray}{GPT-Neo-1.3B, BLIP2-opt-2.7B}}                       & \multicolumn{1}{c|}{\textcolor{lightgray}{Text}}                      & \textcolor{lightgray}{0.695}                   & \multicolumn{1}{l|}{\textcolor{lightgray}{0.650}} & \multicolumn{1}{c}{\textcolor{lightgray}{-}}                        & \multicolumn{1}{c}{\textcolor{lightgray}{-}}                        & \multicolumn{1}{c|}{\textcolor{lightgray}{-}}      \\ \hline
% \multicolumn{1}{|l||}{Video LLM~\cite{chen2023videollm}}               & \multicolumn{1}{l|}{GPT-2}                       & \multicolumn{1}{c|}{Video}                     & 0.721                    & \multicolumn{1}{l|}{0.725}  & \multicolumn{1}{c}{-}                        & \multicolumn{1}{c}{-}                        & \multicolumn{1}{c|}{0.154}  \\ 
% \multicolumn{1}{|l||}{Video LLAMA~\cite{zhang2023video}}             & \multicolumn{1}{l|}{LLaMA2-7B-chat-hf}                       & \multicolumn{1}{c|}{Video}                     &                          & \multicolumn{1}{l|}{}       &                          &                          & \multicolumn{1}{l|}{}       \\ \hline
% \multicolumn{1}{|l||}{\textbf{Ours}}                    & \multicolumn{1}{l|}{LLaMA2-7B-chat-hf}                       & \multicolumn{1}{c|}{Video}                     &                          & \multicolumn{1}{l|}{}       &                          &                          & \multicolumn{1}{l|}{}       \\ \hline
% \end{tabular}
% \caption{Performance on Long-term action anticipation on Ego4D $\downarrow$: Lower is better, and \epickitchens on class-mean Top-5 recall~(\%) $\uparrow$): Higher is better}
% \label{tbl:mainego4dek100}
% \end{table*}

==> tables/supp_dnr_ego4d.tex <==
\begin{table}[]
\centering
\begin{tabular}{l|cc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Method}}}               & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}ED@(Z=20) $\downarrow$\end{tabular}}} \\ \cline{2-3} 
\multicolumn{1}{c|}{}                                               & \textbf{Verb}                                & \textbf{Noun}                               \\ \hline
 % Video-LLaMA~\cite{zhang2023video}  & 0.703  & 0.721 \\
\begin{tabular}[c]{@{}l@{}}PlausiVL (w/ DNR)\end{tabular} &  0.689 & 0.695 \\ 
PlausiVL  & 0.679   & 0.681 \\ \hline
\end{tabular}
\caption{(Ego4D)~Performance of \method with and without "DNR: Do NOT repeat actions" in the prompt. We can observe that having DNR in the prompt does not give much improvement in the performance as compared to training the model with long-horizon action repetition loss~($\Lrep$) as objective function.}
\vspace{-2mm}
\label{tbl:dnr_ego4d}
\end{table}

==> tables/supp_dnr_ek100.tex <==
\begin{table}[]
\centering
\begin{tabular}{l|ccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Method}}}          & \multicolumn{3}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Class-mean \\ Top-5 recall (\%) $\uparrow$\end{tabular}}} \\ \cline{2-4} 
\multicolumn{1}{c|}{} & \textbf{Verb}                           & \textbf{Noun}                          & \textbf{Action}                          \\ \hline
 % Video-LLaMA~\cite{zhang2023video} & 52.90 & 52.01 & 26.05 \\
\begin{tabular}[c]{@{}l@{}}PlausiVL (w/ DNR)\end{tabular} & 54.30 & 53.20 & 26.63                                      \\ 
PlausiVL   &   55.62  &  54.23   & 27.60 \\ \hline
\end{tabular}
\caption{(\epickitchens)~Performance of \method with and without "DNR: Do NOT repeat actions" in the prompt. Having DNR in the prompt is less effective than training the model with long-horizon action repetition loss~($\Lrep$) as objective function.}
\vspace{-2mm}
\label{tbl:dnr_ek100}
\end{table}
